Dynamic Automatic Differentiation of GPU Broadcast Kernels

We show how forward-mode automatic differentiation (AD) can be employed within larger reverse-mode computations to dynamically differentiate broadcast operations in a GPU-friendly manner. Our technique fully exploits the broadcast Jacobian's inherent sparsity structure, and unlike a pure reverse-mode approach, this "mixed-mode" approach does not require a backwards pass over the broadcasted operation's subgraph, obviating the need for several reverse-mode-specific programmability restrictions on user-authored broadcast operations. Most notably, this approach allows broadcast fusion in primal code despite the presence of data-dependent control flow. We discuss an experiment in which a Julia implementation of our technique outperformed pure reverse-mode TensorFlow and Julia implementations for differentiating through broadcast operations within an HM-LSTM cell update calculation.

==> img/common.tex <==
\usepackage{pgfplots, pgfplotstable}
\usepgfplotslibrary{units}

% PGF version management
\pgfplotsset{compat=1.13}
\pgfplotsset{compat/show suggested version = false}

% command for filtering rows based on a column value
\pgfkeys{
    /tr/rowfilter/.style 2 args={
        /pgfplots/x filter/.append code={
            \edef\arga{\thisrow{#1}}
            \edef\argb{#2}
            \ifx\arga\argb
            \else
                \def\pgfmathresult{}
            \fi
        }
    }
}

% DataFrames.writetable uses quotes, which PGF doesn't handle
\pgfplotstableset{ignore chars={"}, col sep=comma}

\usepackage{tikz}
\usetikzlibrary{patterns}

